The visibility based Tapered Gridded Estimator (TGE) for the redshifted 21-cm power spectrum

We present the improved visibility based Tapered Gridded Estimator (TGE) for the power spectrum of the diffuse sky signal. The visibilities are gridded to reduce the computation, and tapered through a convolution to suppress the contribution from the outer regions of the telescope's field of view. The TGE also internally estimates the noise bias, and subtracts this out to give an unbiased estimate of the power spectrum. An earlier version of the 2D TGE for the angular power spectrum $C_{\ell}$ is improved and then extended to obtain the 3D TGE for the power spectrum $P({\bf k})$ of the 21-cm brightness temperature fluctuations. Analytic formulas are also presented for predicting the variance of the binned power spectrum. The estimator and its variance predictions are validated using simulations of $150 \, {\rm MHz}$ GMRT observations. We find that the estimator accurately recovers the input model for the 1D Spherical Power Spectrum $P(k)$ and the 2D Cylindrical Power Spectrum $P(k_\perp,k_\parallel)$, and the predicted variance is also in reasonably good agreement with the simulations.

==> readme <==
%auto-ignore

This file contain information regarding the paper "The visibility based Tapered Gridded Estimator (TGE) for the redshifted 21-cm power spectrum"

Authors:Samir Choudhuri, Somnath Bharadwaj, Suman Chatterjee, Sk. Saiyad Ali, Nirupam Roy, and Abhik Ghosh

Comments: 19 pages, 13 figures. Accepted for publication in MNRAS. The definitive version will be available at http://mnrasl.oxfordjournals.org/

The contact details of the first author are as follows
Samir Choudhuri
email  : samir11@phy.iitkgp.ernet.in
Address: Indian Institute of Technology Kharagpur
         Kharagpur-721302, India



Abstract:We present the improved visibility based Tapered Gridded Estimator (TGE) for
the power spectrum of the diffuse sky signal.  The visibilities are
gridded to reduce the computation, and tapered through a convolution
to suppress the contribution from the outer regions of the
telescope's field of view.  The TGE also internally estimates the
noise bias, and  subtracts this out to give an unbiased
estimate of the power spectrum. An earlier version of the 2D TGE for
the angular power spectrum $C_{\ell}$ is improved and then extended to
obtain the 3D TGE for the power spectrum $P({\bf k})$ of the 21-cm
brightness temperature fluctuations. Analytic formulas are also
presented for predicting the variance of the binned power spectrum.
The estimator and its variance predictions are validated using
simulations of $150 \, {\rm MHz}$ GMRT observations.  We find that the
estimator accurately recovers the input model for the 1D Spherical
Power Spectrum $P(k)$ and the 2D Cylindrical Power Spectrum
$P(k_\perp,k_\parallel)$, and the predicted variance is also in
reasonably good agreement with the simulations.

The compressed tar file "tgepk_3_arxiv.tar.gz" contain the following files:

readme : This file
ms.tex : Manuscript file in LaTeX format
mn2e.cls : Manuscript class file
fig01.ps      :Fig 1 (Colour for online)
fig1acolor.ps : Fig 2(a) (Colour for online)
fig1bcolor.ps : Fig 2(b) (Colour for online)
fig1aacolor.ps : Fig 3(a) (Colour for online)
fig1bbcolor.ps : Fig 3(b) (Colour for online)
fig2acolor.ps : Fig 4(a) (Colour for online)
fig2bcolor.ps : Fig 4(b) (Colour for online)
binning_sphere.eps: Fig 5(a) (Colour for online)
binning_cylinder.eps: Fig 5(b) (Colour for online)
fig5acolor.ps : Fig 6(a) (Colour for online)
fig5bcolor.ps : Fig 6(b) (Colour for online)
fig6acolor.ps : Fig 7(a) (Colour for online)
fig6bcolor.ps : Fig 7(b) (Colour for online)
fig7acolor.ps : Fig 8(a) (Colour for online)
fig7bcolor.ps : Fig 8(b) (Colour for online)
fig8acolor.ps : Fig 9(a) (Colour for online)
fig8bcolor.ps : Fig 9(b) (Colour for online)
fig9acolor.ps : Fig 10(a) (Colour for online)
fig9bcolor.ps : Fig 10(b) (Colour for online)
fig9ccolor.ps : Fig 10(c) (Colour for online)
fig9aacolor.ps : Fig 11(a) (Colour for online)
fig9bbcolor.ps : Fig 11(b) (Colour for online)
fig10acolor.ps : Fig 12(a) (Colour for online)
fig10bcolor.ps : Fig 12(b) (Colour for online)
fig10ccolor.ps : Fig 12(c) (Colour for online)
fig10dcolor.ps : Fig 12(d) (Colour for online)
fig10aacolor.ps : Fig 13(a) (Colour for online)
fig10bbcolor.ps : Fig 13(b) (Colour for online)

